VeriDebug: A Unified LLM for Verilog Debugging via Contrastive Embedding and Guided Correction

Large Language Models (LLMs) have demonstrated remarkable potential in debugging for various programming languages. However, the application of LLMs to Verilog debugging remains insufficiently explored. Here, we present VeriDebug, an approach that integrates contrastive representation and guided correction capabilities for automated Verilog debugging. Unlike existing methods, VeriDebug employs an embedding-based technique to accurately retrieve internal information, followed by bug-fixing. VeriDebug unifies Verilog bug detection and correction through a shared parameter space. By simultaneously learning bug patterns and fixes, it streamlines debugging via contrastive embedding and guided correction. Empirical results show the efficacy of VeriDebug in enhancing Verilog debugging. Our VeriDebugLoc, Type model achieves 64.7 accuracy in bug fixing (Acc1), a significant improvement from the existing open-source SOTAs 11.3. This performance not only outperforms open-source alternatives but also exceeds larger closed-source models like GPT-3.5-turbo (36.6), offering a more accurate alternative to conventional debugging methods.

==> tables/tasks.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{array}
% \usepackage{booktabs}
\begin{table*}[htbp]
\centering
\begin{threeparttable}
\setlength{\tabcolsep}{4pt}
\renewcommand\arraystretch{1.2}
\caption{Task Types, Instructions, and Model Responses for \ours{} training.}
\begin{tabular}{p{1.2cm}p{1.8cm}p{5.5cm}p{5.5cm}}
\toprule
\textbf{Type} & \textbf{Task} & \textbf{Instruction} & \textbf{Response} \\
\specialrule{.08em}{.2em}{.2em} 
\multirow{1}{*}{Embedding} & Line location & Find the buggy line in the code segment. & Positive (Buggy line): 

\texttt{assign adder\_out = rs1\_data;}
 
Negative (Irrelevant lines): 

\texttt{always \@(posedge clk) begin}, 

\texttt{wire [23:0]  sign\_s;},

\texttt{tDst = srca >> tSh;}, 

\texttt{...}\\
\cmidrule(l){2-4}
 & Classification & Infer the bug type in the code segment. & Positive (Bug class): 

\texttt{The bug type is width.}
 
Negative (Wrong bug classes): 

\texttt{The bug type is assignment.}, 

\texttt{The bug type is bitwidth.},

\texttt{The bug type is assignment.}, 

\texttt{...}\\ 
\midrule
Generative & Fix & Your task is to return a JSON to analyze how the code should be modified, in the following format:
\{
    "buggy\_code": "The buggy code in the 
                 SystemVerilog (just one 
                 line of code)",
    "correct\_code": "The correct code (just 
                   one line that can directly 
                   replace the buggy code, 
                   without any other 
                   description)"
\} & \{

"buggy\_code": 

\texttt{assign data\_s = (type\_s == 1'b1) ? {~data[DW], data[(DW-1):0]} : data;}

"correct\_code": 

\texttt{assign data\_s = (type\_s == 1'b0) ? {~data[DW], data[(DW-1):0]} : data;}

\}
\\
\bottomrule
\end{tabular}
\label{tab:task}
\end{threeparttable}
\end{table*}

